MAGE: Mutual Attestation for a Group of Enclaves without Trusted Third Parties

Intel Software Guard Extensions (SGX) local and remote attestation mechanisms enable an enclave to attest its identity (i.e., the enclave measurement, which is the cryptographic hash of its initial code and data) to an enclave. To verify that the attested identity is trusted, one enclave usually includes the measurement of the enclave it trusts into its initial data in advance assuming no trusted third parties are available during runtime to provide this piece of information. However, when mutual trust between these two enclaves is required, it is infeasible to simultaneously include into their own initial data the other's measurements respectively as any change to the initial data will change their measurements, making the previously included measurements invalid. In this paper, we propose MAGE, a framework enabling a group of enclaves to mutually attest each other without trusted third parties. Particularly, we introduce a technique to instrument these enclaves so that each of them could derive the others' measurements using information solely from its own initial data. We also provide a prototype implementation based on Intel SGX SDK, to facilitate enclave developers to adopt this technique.

==> tex/071-alternative.tex <==
\section{Comparison to Alternatives}

\subsection{A Straw-man Solution}

\yz{Can we drop this strawman solution all together??}


%\subsection{Merging Enclaves to Form the Same Measurement}
A straw-man solution leverages the fact that one enclave could obtain its own measurement during runtime, \eg, by calling \texttt{EREPORT} to get a report which includes a field filled with its own measurement by the SGX implementation. Hence, when receiving a quote or report, an enclave could verify the identity of the attester by comparing the measurement filed in the quote or report against its own measurement. %has the same measurement as the target enclave, the target enclave could produce its own measurement for verification. 

%\bheading{Enclave Modification.} 
Consider a group of two enclaves  \isve{1} (with content $C_1$) and \isve{2} (with content $C_2$), enclave developers combine the two enclaves into one single enclave \isve{(1,2)} (with content $C_1||C_2$). Restrictions can be added to \isve{(1,2)} such that after initialization, either only the components originally from \isve{1}, or the components originally from \isve{2} can be run. For example, a global variable can be used to indicate the identity. % which could only be set once after launching. 
Particularly, consider a global variable called \textit{role} is introduced for this purpose. Its value is initialized to be $0$, which is integrity-protected by the enclave measurement. An enclave API is provided to enable the host program to set the role of the enclave after the enclave is launched. This API should be carefully designed such that \textit{role} could be set only once throughout the whole enclave life cycle. Specifically, its value could  be changed either $1$ or $2$ only when it equals to its initial value, \ie, $0$. And when multiple threads are supported, secure locks need to be adopted to avoid attacks such as AsyncShock~\cite{Weichbrodt:2016:AsyncShock}. After the role is set, before executing any enclave function, the global variable will be checked. If it is set to $1$, the enclave functions originally from \isve{1} within the range of $C_1$ can be run normally while the enclave functions originally from \isve{2} within the range of $C_2$ will abort directly. Hence, one instance of \isve{(1,2)} could only act as \isve{1} (denoted as \isve{(1,2)|1}) or \isve{2} (denoted as \isve{(1,2)|2}).

%\bheading{Measurement Derivation.}
Though \isve{(1,2)|1} and \isve{(1,2)|2} might act differently, they have exactly the same measurement. Hence, \isve{(1,2)|1} could produce \isve{(1,2)|2}'s measurement by simply calling \texttt{EREPORT} and obtaining the measurement from the generated report.

\bheading{Extensions and Limitation.}
This method can be easily extended to a group of enclaves, \isve{1}, \isve{2},\dots, \isve{N}: a unified enclave \isve{(1,2,\dots,N)} that contains all contents of \isve{1}, \isve{2},\dots, \isve{N} is created and restrictions are added such that each instance of the unified enclave could act as only one of $N$ different enclaves, \ie, \isve{(1,2,...,N)|1}, \isve{(1,2,...,N)|2}, \dots, \isve{(1,2,...,N)|N}). They all share the same measurement.
However, this method is not scalable as the size of the unified enclave grows linearly with regards to the number of enclaves. Given that SGX v1 supports a maximum enclave memory of $128$ \mbytes for a single enclave, this method only works for groups of small sizes. Additionally, it might add extra workload for enclave developers to resolve potential conflicts when combining these enclaves into one, \eg, duplicate global variable names and function names.



